Testing and Debugging Techniques for Answer Set Solver Development

This paper develops automated testing and debugging techniques for answer set solver development. We describe a flexible grammar-based black-box ASP fuzz testing tool which is able to reveal various defects such as unsound and incomplete behavior, i.e. invalid answer sets and inability to find existing solutions, in state-of-the-art answer set solver implementations. Moreover, we develop delta debugging techniques for shrinking failure-inducing inputs on which solvers exhibit defective behavior. In particular, we develop a delta debugging algorithm in the context of answer set solving, and evaluate two different elimination strategies for the algorithm.

==> abstract.tex <==
This paper develops automated testing and debugging techniques 
for answer set solver development.
We describe a flexible grammar-based black-box ASP fuzz testing tool 
which is able to reveal various defects
such as unsound and incomplete behavior, i.e.~invalid answer sets and
inability to find existing solutions, in state-of-the-art answer set solver 
implementations.
Moreover, we develop  delta debugging techniques for
shrinking failure-inducing inputs on which solvers exhibit defective
behavior. In particular, we develop a delta debugging algorithm in
the context of answer set solving, 
and evaluate two different elimination strategies for the algorithm.


==> asp.tex <==
\vspace{-.1cm}
\section{Answer Set Programs}
\label{sec:asp}

This section reviews the stable model semantics and the classes of 
answer set programs considered in this work. 

\paragraph{Normal Logic Programs and Answer Sets}
\label{programs}

A normal logic program (NLP) consists of a finite set of
\emph{normal} rules of
the form  
$$r \ : \ h\mIF a_1,\ldots, a_n,\naf b_1,\ldots, \naf b_m,$$
%
where each $a_i$ and $b_j$ is a propositional (or \emph{normal}) 
atom, and $h$ is either
a propositional atom or the symbol $\bot$ that stands for falsity. 
%
A rule $r$ consists of a \emph{head}, $\head(r)=h$, and a \emph{body},
$\body(r) = \{a_1,\ldots,a_n, \naf b_1, \ldots,\naf b_m\}$.
%
A rule $r$ is a \emph{fact} if $\body(r)=\emptyset$, and
an \emph{integrity constraint} if $head(r)=\bot$.
%
The symbol~``$\naf$'' denotes {\em default negation}. 
A {\em default literal} is an atom $a$ or its default negation
$\naf a$. 

For a rule $r$, let
$\body(r)^{+} = \{a_1,\ldots, a_n\}$ and 
$\body(r)^{-} = \{b_1,\ldots,b_m\}$ denote the sets of positive and
negative (default negated) atoms in 
$\body(r)$, respectively.

In ASP, we are interested in \emph{stable models}~\cite{GL88:iclp} (or
\emph{answer sets}) of a program $\prog$. 
%
An \emph{interpretation} $M \subseteq \atoms(\prog)$ 
defines which atoms of $\prog$ are true ($a\in M$) and
which are false ($a\not\in M$).
%
An interpretation $M\subseteq\atoms({\prog})$ satisfies 
a normal rule $r$
if and only if $\body(r)^{+} \subseteq M$ and
$\body(r)^{-} \isect M=\emptyset$ imply $\head(r)\in M$, and hence
$M$ is a \emph{(classical)
model} of $\prog$ if $M$ satisfies all rules in $\prog$.
%
A model $M$ of a program $\prog$ is an answer set of~$\prog$
if and only if there is no model $M' \subset M$ of $\GLred{\prog}{M},$
where 
%
$\GLred{\prog}{M} = \{ \head(r)\mIF
\body(r)^{+}\mid r \in \prog {\rm \; and \; } \body(r)^{-}\isect M=\emptyset\}$
%
is called the \emph{Gelfond-Lifschitz reduct} of $\prog$ with respect
to $M$. 
%
The problem of deciding whether a NLP has an answer set is 
NP-complete.

\paragraph{Weight Constraint Programs}


In order to enable more convenient modeling in ASP, 
extensions of normal programs have been proposed.
Examples of such extensions are what we refer here to as
\emph{weight constraint programs} (WCPs).
%
A \emph{weight atom} is of the form
$$l [a_1 = w_{a_1}, \ldots, a_n = w_{a_n}, 
\naf b_1 = w_{b_1}, \ldots, \naf b_m = w_{b_m}] u,$$ where
each $l_i \in 
\{a_i\}_{1 \leq i \leq n} \cup 
\{\naf b_j\}_{1 \leq j \leq m}$ 
is a default literal, each $w_i$ an integer (the
\emph{weight} of $l_i$), and $u,l$ are integers with $l \leq u$ 
(the \emph{lower} and \emph{upper bound}, respectively).
%
If one of the bounds $u$ and $l$ is omitted, 
this bound is implicitly $\infty$ (for $u$) or  
$-\infty$ (for $l$).
%
A \emph{cardinality atom} is the special case of a weight atom in
which  each literal has weight one. 
%
The variant of cardinality
 atoms in which \emph{both} of $u,l$ are omitted is called a
\emph{choice atom}, that is
 an expression of the form $\{a_1, \ldots, a_n\}$, where each $a_i$
is a normal atom.

A weight constraint rule is of the form
$r \ : \ C_0\mIF C_1,\ldots, C_n$,
where the head 
$C_0$ is a normal, weight, cardinality, choice atom, or $\bot$  
and each $C_i$, $i> 0$ in the body (which can also be empty) is a 
normal, weight, or cardinality literal.
%
We use the term \emph{weight constraint  programs} for the set of
programs that consist of weight constraint rules.
%
Hence NLPs are special cases of weight constraint programs.

Given an interpretation $M$, 
the stable model semantics extends to weight constraint
 programs by defining that
%
a weight atom is 
satisfied by $M$
 if and only if 
$l \leq \sum_{a_i \in M} w_i + \sum_{b_j \not\in M} w_j\leq u$.
 %
A choice atom is always satisfied by $M$.
%
The problem of deciding whether a given weight constraint program
has an answer set remains in NP.

\paragraph{Disjunctive Logic Programs}

Another extension of normal rules are \emph{disjunctive rules}, in
which the head can, instead of a normal atom, be a disjunction $\bigvee_{i=1}^n a_i$ of  normal atoms.
%
Disjunctive logic programs (DLPs)  can contain normal
and disjunctive rules.
%
The stable model semantics extends to the disjunctive case naturally
by defining that
a disjunctive rule $r$ with $\head(r) = \bigvee_{i=1}^n a_i$ is satisfied by 
an interpretation $M$ if and only if $\body(r)^{+}\subseteq M$ and
$\body(r)^{-} \isect M=\emptyset$ imply $a_i \in M$ for some $i$.
%
The problem of deciding whether a DLP has an answer set is 
$\Sigma_2^p$-complete and thus presumably harder than the case of NLPs.



==> conclusions.tex <==
\vspace{-.3cm}
\section{Conclusions}
\label{sec:conclusions}
\vspace{-.1cm}

We developed novel fuzz testing and delta debugging techniques for
answer set solver development.
%
The tools provide black-box solutions
for more rigorous testing of a wide range of answer set solvers.
%
ASP applications heavily depend on the robustness and 
correctness of answer set solvers.
However, our experimental analysis clearly showed that our 
fuzz testing tool is able to reveal a variety of different critical defects 
such as segmentation faults, aborts, infinite loops, incorrect results and 
invalid answer sets in various
state-of-the-art answer set solvers. 
Moreover, we showed that
our delta debugging techniques are very effective in shrinking
failure-inducing inputs, which enables efficient debugging of answer
set solvers.

As an extension of this work, we are particularly interested in
testing and debugging solutions for the non-ground case. As many of
the current state-of-the-art solvers heavily depend on the robustness and
correctness of grounders, we find this an interesting and 
important aspect of future work.


==> defs.tex <==
\DeclareMathSymbol{\naf}{\mathord}{symbols}{"18}

%\newtheorem{theorem}{Theorem}[section] 
%\newtheorem{corollary}[theorem]{Corollary} 
%\newtheorem{definition}[theorem]{Definition} 
%\newtheorem{proposition}[theorem]{Proposition} 
%\newtheorem{lemma}[theorem]{Lemma} 
%\newtheorem{example}[theorem]{Example} 

%\newcommand{\qed}{\hfill $\Box$}
\newcommand{\TRUE}{{\bf T}}
\newcommand{\FALSE}{{\bf F}}
\newcommand{\true}{{\bf t}}
\newcommand{\false}{{\bf f}}
\newcommand{\T}{\mathsf{true}}
\newcommand{\F}{\mathsf{false}}
\newcommand{\TRES}{\mathsf{T\mbox{\sf -}RES}}
\newcommand{\RES}{\mathsf{RES}}
\newcommand{\ERES}{\mathsf{E\mbox{\sf -}RES}}
\newcommand{\EASPT}{\mathsf{E\mbox{\sf -}ASP\mbox{\sf -}T}}
\newcommand{\ASPT}{\mathsf{ASP\mbox{\sf -}T}}

\newcommand{\bbox}{\blacksquare}
\newcommand{\isect}{\cap}
\newcommand{\pair}[2]{\langle{#1},{#2}\rangle}
\newcommand{\sel}[2]{\{{#1}\mid{#2}\}}
\newcommand{\GLred}[2]{{#1}^{#2}}
\newcommand{\mIF}{\leftarrow}
\newcommand{\hb}[1]{\mathrm{Hb}(#1)}
\newcommand{\hbv}[1]{\mathrm{Hb_v}(#1)}
\newcommand{\hbh}[1]{\mathrm{Hb_h}(#1)}
\newcommand{\rsep}{.\;}
\newcommand{\join}{\sqcup}
\newcommand{\lpeq}[1]{\equiv_{\mathrm{#1}}}
\newcommand{\fun}[2]{:{#1}\rightarrow{#2}}
\newcommand{\sm}[1]{\mathrm{SM}(#1)}
\newcommand{\lm}[1]{\mathrm{LM}(#1)}
\newcommand{\module}[1]{\mathbb{#1}}
\newcommand{\bottom}[2]{\mathsf{bottom}(#1,#2)}
\newcommand{\rest}[3]{\mathsf{eval}(\topp{#1}{#2},#3)}
\newcommand{\topp}[2]{\mathsf{top}(#1,#2)}
\newcommand{\dep}[1]{\mathsf{Dep}^+\!(#1)}
\newcommand{\eval}[2]{#1/#2}
\newcommand{\simplify}[3]{\mathrm{simp}(#1,#2,#3)}
\newcommand{\hid}[1]{#1_{\mathrm{h}}}
\newcommand{\vis}[1]{#1_{\mathrm{v}}}
\newcommand{\eqt}{\mathrm{EQT}}
\newcommand{\system}[1]{\textsc{#1}}
\renewcommand{\Join}[2]{\underset{#1}{\overset{#2}{\bigsqcup}}}
\newcommand{\sche}[1]{\mathbf{#1}}
\newcommand{\PHP}{{\rm PHP}_n^{n+1}}
\newcommand{\EXT}{{\rm EXT}^{l}}
\newcommand{\CPHP}{{\rm CPHP}_n^{n+1}}
\newcommand{\EPHP}{{\rm EPHP}_n^{n+1}}
\newcommand{\E}{{\rm E}}
\newcommand{\BODY}{\mathsf{body}}
\newcommand{\LOOP}{\mathsf{loop}}
\newcommand{\eb}{\mathsf{eb}}
\newcommand{\prog}{\Pi}
\newcommand{\lits}{L}
\newcommand{\visible}{\mathsf{v}}
\newcommand{\hidden}{\mathsf{h}}

\newcommand{\red}{\mathsf{red}}
\newcommand{\dlits}{\mathsf{dlit}}
\newcommand{\body}{\mathsf{body}}
\newcommand{\head}{\mathsf{head}}
\newcommand{\rules}{\mathsf{rule}}
\newcommand{\comp}{\mathsf{comp}}
\newcommand{\nlp}{\mathsf{nlp}}
\newcommand{\vars}{\mathsf{var}}
\newcommand{\slits}{\mathsf{lit}}
\newcommand{\clauset}{\mathcal{C}}
\newcommand{\facts}{\mathsf{fact}}
\newcommand{\atoms}{\mathsf{atom}}

\newcommand{\smodels}{\mathsf{smodels}}
\newcommand{\nomore}{\mathsf{noMore}}
\newcommand{\clasp}{\mathsf{clasp}}
\newcommand{\cmodels}{\mathsf{cmodels}}
\newcommand{\dlv}{\mathsf{dlv}}
\newcommand{\assat}{\mathsf{assat}}


==> introduction.tex <==

\section{Introduction}

Answer set programming (ASP)~\cite{GL88:iclp,DBLP:journals/amai/Niemela99}
 is a rule-based declarative programming 
paradigm that has proven to be an effective approach to 
knowledge representation and reasoning in various hard combinatorial 
problem domains. 
This success has been enabled by the development of efficient answer
set solvers~\cite{DBLP:journals/ai/SimonsNS02,DBLP:conf/lpnmr/WardS04,Lin:assat,JN04:lpnmr,DBLP:conf/lpnmr/LiuT05,DBLP:conf/lpar/AngerGLNS05,DBLP:journals/tocl/LeonePFEGPS06,GiunchigliaLM:answer,Janhunen:JANCL,clasp,DBLP:conf/kr/DrescherGGKKOS08,JanhunenNS:LPNMR09,BrainV:JLC}.

Implementing robust, sound and complete answer set solvers is a
demanding task. For achieving high solver performance, one needs
to implement error-prone
and complex inference rules, specialized data structures, and other complex
optimizations.
%
On the other hand, robustness and correctness are two essential 
criteria for answer set solvers. 
The users of answer set solvers  heavily 
depend on correct results and, in particular, correct answer sets.
%
The lack of systematized testing tools
for answer set solver development may leave intricate
implementation bugs unnoticed. Indeed, in practice, 
small sets of problem instances that are typically used during regression
and unit testing are not enough for testing correctness 
during solver development.
%
Moreover, while the availability of standard benchmark instances is
of high importance for benchmarking solver implementations,
testing during solver development should not solely rely on these 
instances.
%
In support of these claims, by examining the detailed results of
 the first and second ASP programming competitions~\cite{DBLP:conf/lpnmr/GebserLNNST07,DBLP:conf/lpnmr/DeneckerVBGT09} one
 notices that, on the sets of (typical) benchmarks used in these
 competition, only very few solvers  on very few benchmarks were judged
 as providing incorrect results. In other words, almost no
 defective behavior seems to have been detected.
%
In contrast, we will show that by using the testing and debugging
techniques developed in this work, various kinds of incorrect and
erroneous behavior can be automatically detected and debugged for various
state-of-the-art answer set solvers; furthermore, this is achieved
without the need for the user to construct hand-crafted benchmarks.
%
The testing techniques developed here provide complementary
means for developing highly correct solvers, which can be applied in
addition to domain-specific benchmarks.
Additionally, our delta debugging techniques
can be naturally applied also when defective
solver behavior is detected on domain-specific benchmarks.


In more detail, this  paper develops domain-specific
\emph{grammar-based black-box fuzz testing} and \emph{delta debugging} 
techniques that
enable more systematic testing and debugging solutions for
answer set solver development.
%
Fuzz testing, also called 
\emph{fuzzing}~\cite{SuttonGA:Fuzzing,TakanenDM:Fuzzing}, 
has its origin in software security and quality assurance.
%
The main idea of fuzzing is to test software against random inputs in order to
find \emph{failure-inducing inputs} that trigger defective behavior.
%
In order to find as many defects as possible, 
a ``good'' \emph{fuzzer} (the input generator) 
should generate a wide variety of different inputs.
%
In the \emph{grammar-based} approach,
the generated input
is guaranteed to be \emph{syntactically} valid, i.e.~the input respects
the expected input format. 
%
In \emph{black-box fuzzing}, testing is performed against the software
interface without access to the implementation details of the software.
%
We develop a black-box grammar-based 
fuzz testing tool that is able to generate random ASP
instances from various different classes.
%

In many cases, randomly generated failure-inducing inputs
may contain
large parts that are irrelevant for triggering defective behavior,
and can hence 
be too large to enable efficient debugging. 
In the context of ASP, a failure-inducing answer set program
can simply have too many rules and atoms for a developer to
manually pinpoint the subset of program rules that triggers the
defective behavior.
%
In order to isolate the failure-inducing parts of
such failure-inducing inputs, an automatic technique called \emph{delta
  debugging}~\cite{ZellerH:Simplifying,Zeller:Why,DBLP:conf/icfp/ClaessenH00,DBLP:conf/icse/Misherghi06} has been proposed.
%
Minimization of the size of 
failure-inducing input is intractable in general, and
hence delta debuggers are based on greedy heuristics.
%
We develop an efficient and novel delta debugger which is very
effective in producing small failure-inducing inputs (answer set
programs), hence relieving
the solver developer from the troublesome task of locating
the typically small failure-inducing parts of a large failure-inducing
answer set program.

\paragraph{Main contributions}
We develop a \emph{grammar-based black-box fuzz testing tool for
  answer set solvers} that
covers
various different classes of grounded answer set programs.
%
Our experimental analysis shows that our fuzzing approach is very effective in
revealing various sources of incorrectness, including both 
unsound and incomplete behavior,
 in a wide range of state-of-the-art answer set solvers.
%
Additionally, of independent interest is that since
 our fuzzer is highly configurable,
it can also be used as a flexible ASP benchmark generator.
%
Moreover, we develop a novel delta debugging algorithm for answer set solver
development. Our algorithm uses the 
hierarchical~\cite{DBLP:conf/icse/Misherghi06} structure of answer set 
programs to shrink failure-inducing instances effectively.
Furthermore, we evaluate two different elimination strategies we have 
implemented for our delta debugging algorithm:
a simple and easy-to-implement ``one-by-one'' elimination strategy, and
another one based on the more intricate 
DDMin algorithm originally proposed in different context~\cite{ZellerH:Simplifying}.

All tools developed in this work are publicly available and can be downloaded
at 
\url{http://fmv.jku.at/fuzzddtools/}.
%
Since the tools treat answer set solvers to be tested as black-box
entities, no modifications to the actual solvers are needed in order
to apply these tools in the development process of any answer set solver that
accepts input in the 
standard \textit{lparse} format.

\medskip

The rest of this paper is organized as follows.
First we review necessary concepts related to answer set programs (Section~\ref{sec:asp}).
%
We then present our  fuzzing approach for testing answer set 
solvers (Section~\ref{sec:fuzztest}), with experimental results of the effectiveness
of the fuzzer (Section~\ref{sec:fuzzexperiments}).
%
Finally, we develop delta debugging strategies in the context of
answer set solving (Section~\ref{sec:deltadebug})
and present an experimental evaluation of our approach (Section~\ref{sec:debugexperiments}),
followed by pointers to related work (Section~\ref{sec:related}).


==> related.tex <==
\vspace{-.1cm}
\section{Related work}
\label{sec:related}
\vspace{-.1cm}

The most closely related  work  is the fuzz testing and delta
debugging approach developed for SMT (satisfiability modulo theories)
solvers in~\cite{BrummayerB:SMT09}.
%
Our work differs in
developing ASP specific fuzzing techniques and, especially,
novel delta debugging techniques and strategies in the context of
answer set solving.
%
In contrast to our generic black-box approach,
solver-specific white-box testing solutions are used in the
development process of the DLV solver~\cite{CalimeriLRV:SEA09dlvtracer}.
%
In the context of inductive logic programming for data mining,
a DDMin-based white-box trace-based delta debugger was 
developed~\cite{TronconJ:WLPE}.

As a final note, we want to stress that 
this work develops debugging techniques for answer set
\emph{solvers}, with the aim of developing and providing automated techniques
for developing correct solvers.
%
While this work focuses on solver testing and debugging,
we note that, when considering applications of ASP, 
another possible source of 
errors is the
\emph{modeling} phase in which errors may be introduced by either on a 
conceptual level  or through bugs in  software 
which generate  answer set programs encoding instances of the
application domain. Incorrect modeling can result in answer set programs the
answer sets of which do not precisely capture the set of solutions to
the original problem instance.
%
Various solutions have been recently proposed
for debugging answer set \emph{programs}~\cite{Brain:debugging,Syrjanen:debugging,DBLP:conf/lpnmr/BrainGPSTW07,DBLP:conf/aaai/GebserPST08} where the aim is to find
explanations on why a set of program rules does not describe a 
correct set of answer sets.

